Automorphisms of K-groups II

This work is a continuation of Automorphisms of $K$-groups I, P. Flavell, preprint. The main object of study is a finite $K$-group $G$ that admits an elementary abelian group $A$ acting coprimely. For certain group theoretic properties $\mathcal P$, we study the $AC_{G}(A)$-invariant $\mathcal P$-subgroups of $G$. A number of results of McBride, 'Near solvable signalizer functors on finite groups' J. Algebra {\bf 78}(1) (1982) 181-214 and 'Nonsolvable signalizer functors on finite groups', J. Algebra {\bf 78}(1) (1982) 215-238 are extended. One purpose of this work is to build a general theory of automorphisms, one of whose applications will be a new proof of the Nonsolvable Signalizer Functor Theorem. As an illustration, this work concludes with a new proof of a special case of that theorem due to Gorenstein and Lyons.

==> lg.tex <==
\section{Local to global results}\label{lg}
We shall generalize some of the results of \ICiteSectionL\
concerning $A$-components to $(A,\fancyP)$-components.
Hence we shall consider the following:
\begin{Hypothesis}\label{lg:1}\mbox{}
    \begin{itemize}
        \item   $r$ is a prime and $A$ is an elementary abelian
                $r$-group that acts coprimely on the $K$-group $G$.

        \item   $\fancyP$ is a group theoretic property that
                satisfies Hypothesis~\ref{pc:1}.

        \item   $H$ is an $A\cz{G}{A}$-invariant subgroup of $G$.
    \end{itemize}
\end{Hypothesis}
%
\noindent It turns out that Hypothesis~\ref{lg:1} is too general
so we shall work with the more restrictive:
\begin{Hypothesis}\label{lg:2}\mbox{}
    \begin{itemize}
        \item   Hypothesis~\ref{lg:1}.

        \item   Whenever $A$ acts coprimely on the $K$-group $X$
                and $\cz{X}{A}$ is a $\fancyP$-group then $X$ is solvable.
    \end{itemize}
\end{Hypothesis}

\begin{Lemma}\label{lg:3}\mbox{}
    \begin{enumerate}
        \item[(a)]  Assume Hypothesis~\ref{lg:1}.
                    If $\fancyP$ is any of the properties
                    ``is trivial'', ``is nilpotent'' or ``has odd order''
                    then Hypothesis~\ref{lg:2} is satisfied.

        \item[(b)]  Assume Hypothesis~\ref{lg:2}.
                    Then every $\fancyP$-group is solvable.
    \end{enumerate}
\end{Lemma}
\begin{proof}
    (a). This follows from \ICiteTheoremKfour.

    (b). Let $X$ be a $\fancyP$-group and let $A$ act trivially on $X$.
\end{proof}

\noindent The main result of this section is the following.
\begin{Theorem}\label{lg:4}
    Assume Hypothesis~\ref{lg:2}
    and suppose $K \in \comp{A,\fancyP}{H}$.
    \begin{enumerate}
        \item[(a)]  There exists a unique $\widetilde{K} \in \compasol{G}$
                    with $K \leq \widetilde{K}$.

        \item[(b)]  Suppose that $H$ is $\cz{G}{a}$-invariant for some $a \in A\nonid$
                    and that $K = [K,a]$.
                    Then $K = \widetilde{K}$.
    \end{enumerate}
\end{Theorem}
\noindent At the end of the section,
examples will be constructed to demonstrate that Theorem~\ref{lg:4}
does not hold under the weaker Hypothesis~\ref{lg:1}.

We work towards proving Theorem~\ref{lg:4} via a sequence of lemmas.

\begin{Lemma}\label{lg:5}
    Assume Hypothesis~\ref{lg:1}.
    Suppose $K \in \comp{A,\fancyP}{H}$ and that $K \leq \layerr{G}$.
    Then there exists a unique $\widetilde{K} \in \comp{A}{G}$
    with $K \leq \widetilde{K}$.
\end{Lemma}
\begin{proof}
    Uniqueness is clear since distinct elements of $\comp{A}{G}$
    have solvable intersection.
    Note that since $H$ is $\cz{G}{A}$-invariant we have
    $K \in \comp{A,\fancyP}{H\cz{G}{A}}$.
    Hence we may assume that $\cz{G}{A} \leq H$.

    Assume the conclusion to be false.
    Let $L \in \comp{A}{G}$.
    Now $L \cap H \subnormal H$ and $K \not\leq L$ so
    Lemma~\ref{ap:4}(d) implies $[K,L \cap H] \leq \op{\fancyP}{K}$.
    As $\cz{L}{A} \leq H$ we have $[K,\cz{L}{A}] \leq \op{\fancyP}{K}$
    and $\cz{L}{A}$ normalizes $K$.
    Since $\cz{\layerr{G}}{A}$ is the product of the subgroups $\cz{L}{A}$
    as $L$ ranges over $\comp{A}{G}$,
    it follows that $[K,\cz{\layerr{G}}{A}] \leq \op{\fancyP}{K}$.

    By hypothesis, $K \leq \layerr{G}$ so $[K,\cz{K}{A}] \leq \op{\fancyP}{K}$.
    Hence $\op{\fancyP}{K}\cz{K}{A} \normal K$ and Coprime Action
    implies that $A$ is fixed point free on $K/\op{\fancyP}{K}\cz{K}{A}$.
    This quotient is therefore solvable by \ICiteTheoremKfour.
    Since $K$ is perfect,
    it follows that $K = \op{\fancyP}{K}\cz{K}{A}$.
    But $[K,\cz{K}{A}] \leq \op{\fancyP}{K}$ so $K/\op{\fancyP}{K}$
    is abelian.
    This contradiction completes the proof.
\end{proof}

\begin{Lemma}\label{lg:6}
    Assume Hypothesis~\ref{lg:2}.
    Then $\op{\fancyP}{H}$ and $\layer{\fancyP}{H}$
    act trivially on $\compp{G}$.
\end{Lemma}
\begin{proof}
    We may suppose that $\cz{G}{A} \leq H$.
    Let $K \in \comp{A}{G}$.
    Now $K$ is nonsolvable,
    so by hypothesis,
    $\cz{K/\zz{K}}{A}$ is not a $\fancyP$-group.
    As $\cz{K}{A} \leq H$ we have $\cz{K}{A} \leq \n{G}{\op{\fancyP}{H}}$
    and also $[\op{\fancyP}{H},\cz{K}{A}]$ is a $\fancyP$-group.
    Lemma~\ref{prel:2} implies that $\op{\fancyP}{H} \leq \n{G}{K}$.

    Next, suppose that $L \in \comp{A,\fancyP}{H}$.
    We claim that $L \leq \n{G}{K}$.
    Now $K \cap H \subnormal H$ so Lemma~\ref{ap:4}(d) implies
    $L \leq K \cap H$ or $[L,K \cap H] \leq \op{\fancyP}{L}$.
    In the first case,
    the claim holds.
    In the second case,
    $[L,\cz{K}{A}]$ is a $\fancyP$-group and Lemma~\ref{prel:2}
    implies $L \leq \n{G}{K}$.

    We have shown that $\op{\fancyP}{H}\layer{\fancyP}{H}$ normalizes $K$.
    Then $A\op{\fancyP}{H}\layer{\fancyP}{H}$ acts on $\compp{K}$
    with $A$ acting transitively.
    \ICiteLemmaPeight\ implies $\op{\fancyP}{H}\layer{\fancyP}{H}$
    acts trivially.
    Since every component of $G$ is contained in an $A$-component,
    the proof is complete.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{lg:4}(a)]
    Since distinct $(A,\mbox{sol})$-components have solvable intersection,
    uniqueness is clear.

    Suppose first that $\sol{G} = 1$.
    Let $N$ be the intersection of the normalizers of the components of $G$.
    Now $\sol{G} = 1$ so $\cz{G}{\layerr{G}} = 1$.
    The Schreier Property implies that $N/\layerr{G}$ is solvable.
    Lemma~\ref{lg:6} implies $K \leq N$ so as $K$ is perfect,
    we have $K \leq \layerr{G}$.
    Apply Lemma~\ref{lg:5}.

    Returning to the general case,
    set $\br{G} = G/\sol{G}$.
    Then $\sol{\br{G}} = 1$ so there exists
    $\br{L} \in \compasol{\br{G}}$ with $\br{K} \leq \br{L}$.
    By Lemma~\ref{ap:4}(j) there exists $M \in \compasol{G}$
    with $\br{L} = \br{M}$.
    Then $K \leq M\sol{G}$.
    Lemma~\ref{ap:4}(i) implies that $M \normal M\sol{G}$
    whence $K = K^{\infty} \leq (M\sol{G})^{\infty} = M$
    and the proof is complete.
\end{proof}

Note that the general Schreier Property as used in the preceding proof
was not listed in the properties of $K$-groups in \cite{I}.
We present an alternative proof that uses only those properties.

\begin{proof}[Alternative proof of Theorem~\ref{lg:4}(a)]
    Assume the result to be false.
    As previously,
    we may suppose that $\sol{G} = 1$ and it suffices to prove
    that $K$ induces a inner automorphisms on each component of $G$.
    Note that as $H$ is $\cz{G}{A}$-invariant,
    we have $K \in \comp{A}{H\cz{G}{A}}$.
    Hence we may assume that $\cz{G}{A} \leq H$.
    Also, $K$ normalizes each component of $G$ by Lemma~\ref{lg:6}.

    Let $L_{0} \in \compp{G}$ and suppose that $[L_{0},K] \not= 1$.
    Set $L = \listgen{L_{0}^{A}} \in \comp{A}{G}$,
    so $[L,K] \not= 1$.
    Now $L \cap H \subnormal H, K \in \comp{A,\fancyP}{H}$
    and $K \not\leq L$,
    so Lemma~\ref{ap:4}(d) implies $[L \cap H,K] \leq \op{\fancyP}{K}$.
    Since $K$ normalizes $L$ we in fact have
    $[L \cap H, K] \leq \op{\fancyP}{K} \cap L$.
    Then $[\cz{L}{A},K] \leq \op{\fancyP}{K} \cap L$
    because $\cz{G}{A} \leq H$.
    As $[L,K] \not= 1$,
    \ICiteTheoremKfour\ implies that $[\cz{L}{A},K] \not= 1$.
    Now $\op{\fancyP}{K}$ is solvable by Lemma~\ref{lg:3}
    so $\op{\fancyP}{K} \cap L$ is a nontrivial $A\cz{L}{A}$-invariant
    solvable subgroup of $L$.
    \ICiteLemmaAQSseven\ implies that $L_{0}$ is isomorphic to
    $\ltwo{2^{r}}, \ltwo{3^{r}}, \uthree{2^{r}}$ or $\sz{2^{r}}$.
    \ICiteTheoremKone\ implies that $\out{L_{0}}$ is solvable,
    which completes the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{lg:4}(b)]
    We may assume that $G = \widetilde{K}$ and also that $\cz{G}{a} \leq H$.
    Suppose first that $\sol{\widetilde{K}} = 1$,
    so $\widetilde{K}$ is $A$-simple.
    Now $K = [K,a]$ so $\cz{G}{a} < H$.
    \ICiteCorollaryAQSnine\ implies $H = \widetilde{K}$.
    As $K \in \comp{A,\fancyP}{H}$ and $\widetilde{K}$ is $A$-simple,
    it follows that $K = \widetilde{K}$.
    Hence we may suppose that $\sol{\widetilde{K}} \not= 1$.

    Set $S = \sol{G}$ and $G^{*} = G/S$.
    Using Coprime Action and the previous paragraph
    we have $K^{*} = \widetilde{K}^{*}$.
    Thus $\widetilde{K} = KS$.
    Now $S \cap H \normal H$ so using Lemma~\ref{ap:4}(d)
    we have $\cz{S}{a} \leq S \cap H \leq \n{G}{K}$.
    Now $K = [K,a]$ so \ICiteLemmaGthree\ implies $S \leq \n{G}{K}$,
    whence $K \normal \widetilde{K} = KS$.
    Since $\widetilde{K}$ is perfect,
    this forces $K = \widetilde{K}$ and completes the proof.
\end{proof}

We close this section with a corollary and an example.
In what follows, \emph{nil} is an abbreviation for the group theoretic
property ``is nilpotent''.

\begin{Corollary}\label{lg:7}
    Let $A$ be an elementary abelian $r$-group that acts coprimely
    on the $K$-group $G$.
    Let $a \in A\nonid$ and suppose that $H$ is an $A\cz{G}{a}$-invariant
    subgroup of $G$.
    \begin{enumerate}
        \item[(a)]  Let $K \in \comp{A}{H}$.
                    Then there exists $\widetilde{K}$ with \[
                        K \leq \widetilde{K} \in \comp{A,\mathrm{nil}}{G}.
                    \]

        \item[(b)]  Let $K \in \comp{A,\mathrm{nil}}{H}$.
                    Then there exists $\widetilde{K}$ with \[
                        K \leq \widetilde{K} \in \compasol{G}.
                    \]
    \end{enumerate}
\end{Corollary}
\begin{proof}
    (a) follows from \ICiteTheoremLone\ and (b) follows from
    Lemma~\ref{lg:3} and Theorem~\ref{lg:4}(a).
\end{proof}

\noindent The following example shows that the corollary cannot be extended
further and that the restriction on $\fancyP$ in Theorem~\ref{lg:4}
is needed.

\begin{Example}
    Let $r$ be a prime and $J_{1}$ be a simple $r'$-group that admits
    an automorphism $a_{1}$ of order $r$ with $\cz{J_{1}}{a_{1}}$ solvable.
    For example $\ltwo{2^{r}}$ or $\sz{2^{r}}$ with $r > 5$.
    Let $K$ be a simple group with order $n$.
    Then $K$ acts on the direct product \[
        D = J_{1}\listgen{a_{1}} \times J_{2}\listgen{a_{2}} %
        \times\cdots\times J_{n}\listgen{a_{n}}
    \]
    permuting the direct factors regularly.
    Set $a = a_{1}a_{2}\cdots a_{n} \in \cz{D}{K}$
    and put $A = \listgen{a}$.
    Let $G$ be the semidirect product \[
        G = (J_{1} \times\cdots\times J_{n}) \rtimes K.
    \]
    Then $a$ acts on $G$ with
    $\cz{G}{a} = (\cz{J_{1}}{a_{1}} \times\cdots\times \cz{J_{n}}{a_{n}})K$.
    Observe that $K$ is contained in an $(A,\mbox{sol})$-component of $\cz{G}{a}$.
    However, the $(A,\mbox{sol})$-components of $G$ are $J_{1},\ldots,J_{n}$,
    none of which contain $K$.
\end{Example}




